Multiple Instance Learning: A Survey of Problem Characteristics and Applications

Multiple instance learning (MIL) is a form of weakly supervised learning where training instances are arranged in sets, called bags, and a label is provided for the entire bag. This formulation is gaining interest because it naturally fits various problems and allows to leverage weakly labeled data. Consequently, it has been used in diverse application fields such as computer vision and document classification. However, learning from bags raises important challenges that are unique to MIL. This paper provides a comprehensive survey of the characteristics which define and differentiate the types of MIL problems. Until now, these problem characteristics have not been formally identified and described. As a result, the variations in performance of MIL algorithms from one data set to another are difficult to explain. In this paper, MIL problem characteristics are grouped into four broad categories: the composition of the bags, the types of data distribution, the ambiguity of instance labels, and the task to be performed. Methods specialized to address each category are reviewed. Then, the extent to which these characteristics manifest themselves in key MIL application areas are described. Finally, experiments are conducted to compare the performance of 16 state-of-the-art MIL methods on selected problem characteristics. This paper provides insight on how the problem characteristics affect MIL algorithms, recommendations for future benchmarking and promising avenues for research.

==> NegativeDistributionTypes.tex <==
\subsection{Types of distributions}
The type of data distribution influences how the algorithms perform. For instance, some algorithm perform better when the data is clustered, or some methods do not yield good result when the data representation is sparse. Moreover, the shape of the negative distribution also influences how algorithms behave. In some problem like CBIR, one seeks to identify a given object in a picture. Depending on the object the background can be very different from one picture to another. For instance, a cat can be found in various house or nature settings. As another example, suppose the browser history of a user is used to find web pages related to a particular subject, all other pages, the negative instances, can concern any subjects. In those cases the negative class is not distributed in a limited number of well defined clusters. Moreover, it can be difficult obtain a representative sampling of the negative class. Some methods deal better with unseen negative instances than others. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Toy Concept
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
        \centering
        \begin{subfigure}[b]{0.30\textwidth}
                \includegraphics[width=\textwidth]{images/WRTC-AUCI.eps}
                \caption{AUC versus witness rate for instance classification.}              
        \end{subfigure}
        %(or a blank line (\\) to force the subfigure onto a new line)        
        \begin{subfigure}[b]{0.30\textwidth}
                \includegraphics[width=\textwidth]{images/WRTC-UARI.eps}
                \caption{Unweigthed average recall versus witness rate for instance classification.}           
        \end{subfigure}
        
     	\centering
        \begin{subfigure}[b]{0.30\textwidth}
                \includegraphics[width=\textwidth]{images/WRTC-AUCB.eps}
                \caption{AUC versus witness rate for bag classification.}              
        \end{subfigure}
\caption{Average performance of the MIL algorithms on the Toy data set with concept negative instances distribution as the witness rate increases.}
\label{fig:WRTC}       
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Toy Uniform
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}
        \centering
        \begin{subfigure}[b]{0.30\textwidth}
                \includegraphics[width=\textwidth]{images/WRTU-AUCI.eps}
                \caption{AUC versus witness rate for instance classification.}              
        \end{subfigure}
        %(or a blank line (\\) to force the subfigure onto a new line)        
        \begin{subfigure}[b]{0.30\textwidth}
                \includegraphics[width=\textwidth]{images/WRTU-UARI.eps}
                \caption{Unweigthed average recall versus witness rate for instance classification.}           
        \end{subfigure}
        
     	\centering
        \begin{subfigure}[b]{0.30\textwidth}
                \includegraphics[width=\textwidth]{images/WRTU-AUCB.eps}
                \caption{AUC versus witness rate for bag classification.}              
        \end{subfigure}
 \caption{Average performance of the MIL algorithms on the Toy data set with uniform negative instance distribution as the witness rate increases.}
\label{fig:WRTU}       
\end{figure}
